AG-LSEC: Audio Grounded Lexical Speaker Error Correction

Speaker Diarization (SD) systems are typically audio-based and operate independently of the ASR system in traditional speech transcription pipelines and can have speaker errors due to SD and/or ASR reconciliation, especially around speaker turns and regions of speech overlap. To reduce these errors, a Lexical Speaker Error Correction (LSEC), in which an external language model provides lexical information to correct the speaker errors, was recently proposed. Though the approach achieves good Word Diarization error rate (WDER) improvements, it does not use any additional acoustic information and is prone to miscorrections. In this paper, we propose to enhance and acoustically ground the LSEC system with speaker scores directly derived from the existing SD pipeline. This approach achieves significant relative WDER reductions in the range of 25-40% over the audio-based SD, ASR system and beats the LSEC system by 15-25% relative on RT03-CTS, Callhome American English and Fisher datasets.

==> introduction.tex <==
\section{Introduction}

Multi-talker speech transcription systems answer the question “Who spoke what and when?” in an audio recording. Though single-talker speech transcription systems have advanced significantly in the recent years, there are still challenges in transcribing and diarizing multi-talker speech due to the regular speaker changes and overlapping speech in natural conversations. Multi-talker transcription systems can be broadly classified in three categories of systems that aim to transcribe and diarize multi-talker speech: 1) Speech/Speaker Separation followed by ASR \cite{von2020end,9413423,paturi22_interspeech,zhao2023mossformer}, 2) Speaker attributed ASR \cite{chang2020end, kanda22_interspeech,shi23d_interspeech,sklyar2021streaming, berger23_interspeech} and 3) Modular ASR \cite{wang2020transformer,yang2022conformer, rekesh2023fast, radford2023robust}, SD systems \cite{park2022review,wang2018speaker,fujita2019end,kinoshita2021integrating, bredin23_interspeech}. 

Speech Separation systems separate speech from multiple speakers into different channels while performing ASR individually on these channels, thus assigning a speaker label to each transcribed word. These systems are usually trained with Permutation Invariant Training (PIT) which constrains the maximum number of speakers it can handle \cite{von2020end,9413423}, and is also prone to duplicated artifacts across channels among other challenges to handle long-form audio \cite{paturi22_interspeech}. Speaker attributed ASR (SA-ASR) systems either follow PIT based training \cite{sklyar2021streaming, berger23_interspeech} which have the same challenges as above or the more recent Serialized Output Training (SOT) \cite{kanda22_interspeech,shi23d_interspeech}  systems which outputs transcripts of each speaker sequentially. Main drawbacks with SOT systems are the lack of timestamps for the speaker turns needed for downstream applications, and the difficulty of speaker reconciliation across transcribed blocks for long-form audios.  Training both speech separation and SA-ASR systems is data intensive and needs large amounts of multi-channel audio data. Such data is difficult to source, especially for domains outside of telephony, and could also increase cost significantly. Finally, independent modular ASR and SD systems are one of the most successful and practical ways to transcribe multi-talker audios. The ASR and SD systems operate independently and their results are reconciled to assign speaker labels to each transcribed word \cite{shafey2019joint}. Such systems can naturally transcribe and diarize long-form audio by operating on independent speech segments without significantly constraining the maximum number of speakers, though these approaches are error-prone around speaker change or overlapping speech regions due to SD or reconciliation errors. 

Most SD systems in literature rely only on acoustic information \cite{wang2018speaker,fujita2019end} to either extract speaker embeddings locally or perform local diarization with End-to-End Neural Diarizaion (EEND) \cite{kinoshita2021integrating, bredin23_interspeech} followed by clustering across segments globally. Reliance on only acoustic information can lead to speaker errors, mainly around the speaker turns and regions of speech overlaps \cite{park2020speaker, xia2022turn}. In addition to the SD errors, speakers can be attributed to the wrong words in the SD-ASR reconciliation phase \cite{paturi23_interspeech} also due to errors solely in ASR word timings. The reconciliation errors may be higher in regions of speech overlap as SD can identify one of the overlapping speakers while ASR can identify words corresponding to a different overlapping speaker. 

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.7\linewidth]{ASR_timing_errors_v2}
%   \caption{Errors in reconciliation of independent SD and ASR systems due to inaccurate ASR timings}
%   \vspace{-1\baselineskip}
% \end{figure}
\begin{figure*}[htp]
  \centering
  \includegraphics[width=0.9\linewidth]{EEND_AG_LSEC.png}
  \vspace{-0.5\baselineskip}
  \caption{(a) AG-LSEC with Late Fusion of Speaker Scores, (b) Speaker Scores Extraction form the SD pipeline, (c) AG-LSEC with Early Fusion of Speaker Scores}
  \vspace{-1\baselineskip}
\end{figure*}

Lexical information often contains complementary information which can be useful in accurately assigning speaker labels to the transcribed words \cite{park2020speaker, xia2022turn, shafey2019joint}. For instance, analyzing only the written transcript of a conversation, "how are you i am good", enables us to
infer that there is likely a speaker change between the utterances "how are you" and "i am good". There have been few works which leverage lexical information to perform Speaker Diarization. \cite{park2020speaker} leverages lexical information in the clustering phase while \cite{xia2022turn} leverages lexical information in predicting speaker turns prior to embedding extraction and clustering. Though these methods show good DER improvements, these approaches are still prone to ASR reconciliation errors around speaker turns and overlapped speech similar to the other approaches above. Also, both these works need ASR before performing diarization thus increasing the latency of the system. 
%[] models ASR and SD jointly and can take care of such errors but are confined to 2 speaker cases with distinct roles. 

A more recent work which leverages lexical information to correct speaker errors post ASR reconciliation was the LSEC model introduced in \cite{paturi23_interspeech}. It applies an external language model to the ASR transcriptions and fuses these with speaker labels from SD to efficiently correct speaker and reconciliation errors around speaker turns and overlapping speech regions and was shown to improve reconciled SD performance. One shortcoming of this model is that it overly relies on lexical information, which leads to both under-corrections and over-corrections (as demonstrated in Section 3). In this work, we propose to enhance this SEC approach by grounding the model with acoustic information extracted from the speaker diarization module.
